Enhancing Cognitive Diagnosis using Un-interacted Exercises: A Collaboration-aware Mixed Sampling Approach

Cognitive diagnosis is a crucial task in computational education, aimed at evaluating students' proficiency levels across various knowledge concepts through exercises. Current models, however, primarily rely on students' answered exercises, neglecting the complex and rich information contained in un-interacted exercises. While recent research has attempted to leverage the data within un-interacted exercises linked to interacted knowledge concepts, aiming to address the long-tail issue, these studies fail to fully explore the informative, un-interacted exercises related to broader knowledge concepts. This oversight results in diminished performance when these models are applied to comprehensive datasets. In response to this gap, we present the Collaborative-aware Mixed Exercise Sampling (CMES) framework, which can effectively exploit the information present in un-interacted exercises linked to un-interacted knowledge concepts. Specifically, we introduce a novel universal sampling module where the training samples comprise not merely raw data slices, but enhanced samples generated by combining weight-enhanced attention mixture techniques. Given the necessity of real response labels in cognitive diagnosis, we also propose a ranking-based pseudo feedback module to regulate students' responses on generated exercises. The versatility of the CMES framework bolsters existing models and improves their adaptability. Finally, we demonstrate the effectiveness and interpretability of our framework through comprehensive experiments on real-world datasets.

==> AnonymousSubmission/LaTeX/Experiment_tables/cluster.tex <==

\begin{table}[]
%\captionsetup[table]{skip=20pt} % 设置大表标题与表格的垂直间距
%\captionsetup[subtable]{skip=1pt} % 设置子表标题与子表的垂直间距
 \centering

\begin{subtable}{1\linewidth}
\centering
 \caption*{(a) ASSIST}
  \label{assist_cluster}
\resizebox{0.95\textwidth}{!}{%

\begin{tabular}{l|c|c|c}
\hline
            & ACC              & RMSE             & AUC              \\ \hline
cluster=0   & 72.66\%          & 42.94\%          & 76.16\%          \\ \hline
cluster=50  & \textbf{72.89\%} & \textbf{42.83\%} & \textbf{76.23\%} \\ \hline
cluster=100 & 72.76\%          & 42.86\%          & 76.19\%          \\ \hline
cluster=150 & 72.67            & 42.89\%          & 76.10\%          \\ \hline
cluster=200 & 72.59\%          & 42.92\%          & 75.95\%          \\ \hline
  \end{tabular}%
}
 \end{subtable}%
 
  \vspace{0.2cm} % 添加垂直间距

\begin{subtable}{1\linewidth}
\centering
 \caption*{(b) MATH}
  \label{assist_cluster}
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{l|c|c|c}
\hline
            & ACC              & RMSE             & AUC              \\ \hline
cluster=0   & 74.88\%          & 40.71\%          & 78.74\%          \\ \hline
cluster=20  & \textbf{74.93\%} & \textbf{40.53\%} & \textbf{78.81\%} \\ \hline
cluster=50  & 74.81\%          & 40.61\%          & 78.76\%          \\ \hline
cluster=80  & 74.69\%          & 40.70\%          & 78.71\%          \\ \hline
cluster=100 & 74.32\%          & 40.81\%          & 78.65\%          \\ \hline
\end{tabular}%
}
   \end{subtable}%
\end{table}


==> AnonymousSubmission/LaTeX/Experiment_tables/vs_random.tex <==

\begin{figure}[!t]
    \centering
    \begin{subfigure}{1\columnwidth}
        \includegraphics[width=\linewidth]{ASSIST.png}
        \caption{ASSISTments}
    \end{subfigure}
    \begin{subfigure}{1\columnwidth}
        \includegraphics[width=\linewidth]{MATH.png}
        \caption{ MATH}
    \end{subfigure}
    \caption{Sampling Strategy VS. Random Sampling}
    \label{random_experiment}
\end{figure}

